Measure rigidity for random dynamics on surfaces and related skew products

Given a surface $M$ and a Borel probability measure $\nu$ on the group of $C^2$-diffeomorphisms of $M$, we study $\nu$-stationary probability measures on $M$. We prove for hyperbolic stationary measures the following trichotomy: either the stable distributions are non-random, the measure is SRB, or the measure is supported on a finite set and is hence almost-surely invariant. In the proof of the above results, we study skew products with surface fibers over a measure preserving transformations equipped with a decreasing sub-$\sigma$-algebra $\hat {\mathcal F}$ and derive a related result. A number of applications of our main theorem are presented.

==> fig1.tex <==
	\begin{figure}[h]
							\psscalebox{1 } % Change this value to rescale the drawing.
							{
							\psset{unit=.7cm}
							\begin{pspicture}(1,-3.)(9,3.9)
							\def\dsz{5pt}
							\def\lwd{1.5pt}
							\def\labsizea{\small}
							\def\labsizeb{\small}
							
							\psbezier[linecolor=black, linewidth=\lwd](1.4629215,3.1114335)(1.6629214,2.4314334)(1.7429215,1.9314334)(1.8629215,1.3114334)(1.9829215,0.6914334)(1.9629215,-0.56856656)(1.8629673,-1.2977484)(1.7629215,-2.0085666)(1.6829214,-2.5885665)(1.2629215,-3.0885665)
							\psbezier[linecolor=black, linewidth=\lwd](6.4629216,3.1114335)(6.3429213,2.5318358)(6.1829214,2.0703642)(6.2029214,1.0849818)(6.2229214,0.09959931)(6.382921,-0.46366644)(6.4629216,-1.2885666)(6.5429215,-2.1418538)(6.4829216,-2.6400597)(6.2629213,-3.1085665)
							\psbezier[linecolor=darkgray,linestyle=dashed, linewidth=\lwd](9.062922,-2.0885665)(8.262921,-1.9285666)(7.862921,-1.8885666)(6.4629216,-1.2885666)(5.0629215,-0.68856657)(2.8629215,0.7114334)(1.8629215,1.3114334)(0.8629215,1.9114335)(0.84292144,1.9714334)(0.042921446,2.5714333)
							
							
							\psbezier[linecolor=black, linewidth=\lwd](0.0033587317,-1.4236704)(0.7227816,-1.3011878)(0.86325127,-1.2739145)(1.8629673,-1.2977484)(2.862683,-1.3215824)(5.373685,-1.370877)(6.462944,-1.2831012)(7.5522027,-1.1953255)(8.361149,-0.93571675)(9.040381,-0.75355273)
							
							\psbezier[linecolor=darkgray,linestyle=dashed, linewidth=\lwd]
							(4.4629677,-2.3885665)
							(3.6629667,-1.9285666)
							(3.2629667,-1.8885666)
							(1.8629673,-1.2977484)% x  		%(6.4629216,-1.2885666)
							(1.8629673,-1.2977484)% x  		%(6.4629216,-1.2885666)
							(1, -.8)
							(0.0033587317,-.4236704)
							%(-3.7370328, 1.9114335)
							%(-3.75703286, 1.9714334)
							%(-4.557032854, 2.5714333)
							
							
							
							\psdots[linecolor=black, dotsize=\dsz](1.8629673,-1.2977484)%(1.8629215,-1.2885666)
							\psdots[linecolor=black, dotsize=\dsz](6.4629216,-1.2885666)
							\psdots[linecolor=black, dotsize=\dsz](1.8629215,1.3114334)
							
							\uput[45](1.8629673,-1.2977484){\labsizea$x$}
							\uput[45](6.4629216,-1.2885666){\labsizea$y_j$}
							\uput[45](1.8629215,1.3114334){\labsizea$z_j$}
							
							\uput[0](9.040381,-0.75355273){\labsizeb $W^s_\xi(x)$}
							\uput[-15](9.062922,-2.0885665){\labsizeb$W^s_\eta(y_j)$}
							\uput[-15](4.4629677,-2.3885665){\labsizeb$W^s_\eta(x)$}
							%\uput[270](6.2629213,-3.1085665){\labsizeb$W^u_\xi(y_j) =W^u_\xi(y_j)$ }
							\uput[90](6.4629216,3.1114335){\labsizeb$W^u_\xi(y_j) =W^u_\eta(y_j)$ }
							\uput[90](1.4629215,3.1114335){\labsizeb$W^u_\xi(x) =W^u_\eta(x)$ }
							
							\end{pspicture}
							}
							\caption{Choice of $z_j$}\label{fig:1}
							\end{figure}
